An index for unitarizable $\mathfrak{sl}(m\vert n)$-supermodules

The "superconformal index" is a character-valued invariant attached by theoretical physics to unitary representations of Lie superalgebras, such as $\mathfrak{su}(2,2\vert n)$, that govern certain quantum field theories. The index can be calculated as a supertrace over Hilbert space, and is constant in families induced by variation of physical parameters. This is because the index receives contributions only from "short" irreducible representations such that it is invariant under recombination at the boundary of the region of unitarity. The purpose of this paper is to develop these notions for unitarizable supermodules over the special linear Lie superalgebras $\mathfrak{sl}(m\vert n)$ with $m\ge 2$, $n\ge 1$. To keep it self-contained, we include a fair amount of background material on structure theory, unitarizable supermodules, the Duflo-Serganova functor, and elements of Harish-Chandra theory. Along the way, we provide a precise dictionary between various notions from theoretical physics and mathematical terminology. Our final result is a kind of "index theorem" that relates the counting of atypical constituents in a general unitarizable $\mathfrak{sl}(m\vert n)$-supermodule to the character-valued $Q$-Witten index, expressed as a supertrace over the full supermodule. The formal superdimension of holomorphic discrete series $\mathfrak{sl}(m\vert n)$-supermodules can also be formulated in this framework.

==> hacks.tex <==
\makeatletter

%%%
%%%%%% More space in Abstract an Tableofcontents
%%%%%%%%%

\renewenvironment{abstract}{%
  \ifx\maketitle\relax
    \ClassWarning{\@classname}{Abstract should precede
      \protect\maketitle\space in AMS document classes; reported}%
  \fi
  \global\setbox\abstractbox=\vtop \bgroup
    \normalfont\Small
    \list{}{\labelwidth\z@
      \leftmargin3pc \rightmargin\leftmargin
      \listparindent\normalparindent \itemindent\z@
      \parsep\z@ \@plus\p@
      \let\fullwidthdisplay\relax
    }%
    \item[\hskip\labelsep\scshape\abstractname.]%
}{%
  \endlist\egroup
  \ifx\@setabstract\relax \@setabstracta \fi
}

%%%
%%%%%% small big symbols
%%%%%%%%%

\newcommand{\makesmalleroperator}[1]{%
  \expandafter\let\csname saved\string#1\endcsname#1% save the old command
  \def#1{\mathop{\small@mathchoice#1}}% redefine it
}
\def\small@mathchoice#1{%
  \mathchoice{\text{\raisebox{0.25ex}{\scalebox{0.8}{$\@nameuse{saved\string#1}$}}}}%
             {\@nameuse{saved\string#1}}%
             {\@nameuse{saved\string#1}}%
             {\@nameuse{saved\string#1}}%
}

\makesmalleroperator\bigwedge
\makesmalleroperator\bigoplus
\makesmalleroperator\bigotimes




%%%
%%%%%% horizontal lines in arrays
%%%%%%%%%

\newcommand\tstrut{\rule[0ex]{0pt}{2.2ex}}

%%%
%%%%%% sectioning
%%%%%%%%%

\renewcommand\subsubsection{\@startsection{subsubsection}{4}{\z@}% 
                                   {-1.25ex\@plus -1ex \@minus -.2ex}% 
                                   {-1.2ex \@plus .2ex}% 
                                   {\normalfont\normalsize\it}} 

%%%
%%%%%% margin notes
%%%%%%%%%

\def\revise#1{\raisebox{-0em}{\rule{3pt}{1em}}% 
              \marginpar{\raisebox{.5em}{\vrule width3pt\ 
               \vrule width0pt height 0pt depth0.5em 
                \hbox to 0cm{\hspace{1.4cm}{% 
                \parbox[t]{5em}{\raggedright\footnotesize{#1}}}\hss}}}} 

%%%
%%%%%% Bibliography
%%%%%%%%%

%%% this saves a bit of space
\renewcommand*{\bibsetup}{%
  \interlinepenalty=5000\relax
  \widowpenalty=10000\relax
  \clubpenalty=10000\relax
  \raggedbottom
  \frenchspacing
  \biburlsetup
  \renewcommand\baselinestretch{1}
}
\renewcommand{\bibfont}{\fontsize{9pt}{11pt}\selectfont}
\setlength\bibitemsep{.1em}
\setlength\bibhang{0em}
\setlength\biblabelsep{.7em}

%%% this suppresses the In: 
\renewbibmacro{in:}{}
\DeclareFieldFormat{doilink}{%
  \iffieldundef{doi}%
  {#1}%
  {\href{https://doi.org/\thefield{doi}}{#1}}
}
%%% and puts doi link around journal reference
%%% (hacked from standard.bbx https://ctan.org/tex-archive/macros/latex/contrib/biblatex/latex/bbx?lang=en)
\DeclareBibliographyDriver{article}{%
  \usebibmacro{bibindex}%
  \usebibmacro{begentry}%
  \usebibmacro{author/translator+others}%
  \setunit{\printdelim{nametitledelim}}\newblock
  \usebibmacro{title}%
  \newunit
  \printlist{language}%
  \newunit\newblock
  \usebibmacro{byauthor}%
  \newunit\newblock
  \usebibmacro{bytranslator+others}%
  \newunit\newblock
  \printfield{version}%
  \newunit\newblock
  \usebibmacro{in:}
  \iffieldundef{journaltitle}
   {\printtext[journaltitle]{Preprint} \mkbibparens{\printdate}}
   {\printtext[doilink]{%
    \usebibmacro{journal+issuetitle}%
    \newunit
    \usebibmacro{byeditor+others}%
    \newunit
    \usebibmacro{note+pages}%
    \newunit\newblock
    \iftoggle{bbx:isbn}
      {\printfield{issn}}
      {}%
   }
   }
  \newunit\newblock
  \usebibmacro{doi+eprint+url}
  \newunit\newblock
  \usebibmacro{addendum+pubstate}%
  \setunit{\bibpagerefpunct}\newblock
  \usebibmacro{pageref}%
  \newunit\newblock
  \iftoggle{bbx:related}
    {\usebibmacro{related:init}%
     \usebibmacro{related}}
    {}%
  \usebibmacro{finentry}}

%%% this puts brackets around arxiv if journal exists
\letbibmacro{nakedEprint}{eprint}
\renewbibmacro*{eprint}{%
  \iffieldundef{eprint}
    {}
    {\iffieldundef{journaltitle}
      {\usebibmacro{nakedEprint}}
      {\printtext{{\usebibmacro{nakedEprint}}}}} %\mkbibbrackets I think there are too many brackets
}
%%% and changes format of [eprint:arxiv]
%%% (hacked from: https://packages.oth-regensburg.de/ctan/macros/latex/contrib/biblatex/latex/biblatex.def)
\DeclareFieldFormat{eprint:arxiv}{%
  \ifhyperref
    {\href{https://arxiv.org/\abx@arxivpath/#1}{%
       \nolinkurl{arXiv:#1}%
       \iffieldundef{eprintclass}
         {}
         {\addspace{\mkbibbrackets{\thefield{eprintclass}}}}}}  %%% remmoved \texttt
    {\nolinkurl{arXiv:#1}%
     \iffieldundef{eprintclass}
       {}
       {\addspace{\mkbibbrackets{\thefield{eprintclass}}}}}}   %%% removed \texttt

\makeatother
